NRCL - A Model Building Approach to the Bernays-Sch\"onfinkel Fragment (Full Paper)

We combine constrained literals for model representation with key concepts from first-order superposition and propositional conflict-driven clause learning (CDCL) to create the new calculus Non-Redundant Clause Learning (NRCL) deciding the Bernays-Sch\"onfinkel fragment. Our calculus uses first-order literals constrained by disequations between tuples of terms for compact model representation. From superposition, NRCL inherits the abstract redundancy criterion and the monotone model operator. CDCL adds the dynamic, conflict-driven search for an atom ordering inducing a model. As a result, in NRCL a false clause can be found effectively modulo the current model candidate. It guides the derivation of a first-order ordered resolvent that is never redundant. Similar to 1UIP-learning in CDCL, the learned resolvent induces backtracking and, by blocking the previous conflict state via propagation, it enforces progress towards finding a model or a refutation. The non-redundancy result also implies that only finitely many clauses can be generated by NRCL on the Bernays-Sch\"onfinkel fragment, which serves as an argument for termination.

==> app/s1-nc/non-cyclic.tex <==
%Non-cyclic Fragment
\section{NRCL for the Non-cyclic Fragment}
In this section, we extend our calculus to the so-called \emph{non-cyclic fragment} of many-sorted 
first-order logic. This fragment corresponds to the signatures with finite Herbrand universe, and 
proved itself a useful extension of the classic {\mEPR} fragment.

Below, we first extend our language with function symbols and define this fragment, then extend 
both our constraint language and our key results. 
We note that the calculus itself needs no new rules or notions, extending the underlying constraint language
and the related operations suffices.
%
\subsection{Preliminaries}
\input{app/s1-nc/ss-prelim}
%
\subsection{Dismatching Constraints}
\input{app/s1-nc/ss-dmc}
%
\subsection{Decision Procedure}
\input{app/s1-nc/ss-results}
%
\subsection{Conclusion}
\input{app/s1-nc/ss-conc}
%


==> app/s1-nc/ss-conc.tex <==
% conclusion
Here, we conclude the section on non-cyclic fragment. We extended our language with sorts and function symbols, and introduced the necessary notions and notations
to handle the new setting.
We defined the non-cyclic fragment first implicitly, then explicitly using dependency graphs. 

We showed that our calculus extends to this fragment seamlessly, preserving all its properties and our key results for soundness, termination, and non-redundant 
clause learning.

As a final note, we only make the remark that the technical aspects are still to be investigated. In particular, naive grounding is getting more expensive and 
less feasible as we extend our language. Thus, free variable elimination requires further considerations.
%

==> app/s1-nc/ss-dmc.tex <==
% DMC for NcF
\paragraph{Definitions.}
Implicit generalizations were originally designed for the richer first-order language. Thus,
the basic definitions for dismatching constraints and their semantics of Section 2 extend to 
the non-cyclic fragment in a straightforward manner. 
In the extended definition, we assume that every dismatching constraint is well-sorted, \ie the left-hand side and 
right-hand side terms and variables at the same position in the tuples of an atomic constraint have
the same sort.

Due to the generic formulations, all properties in Section 2 follow from the definitions.
In particular, the definition of induced substitutions remains the same, and the 
key property formulated in Remark~\ref{a-inducedsubst-remark} still holds.
We define normal form and constrained expressions analogously to the {\mEPR} case, and 
the extended rule system for normalization is given below.
%
\paragraph{Normalization.}
The original normal form transformation is still suitable, we only have to modify the first three 
rules and add a new rule for decomposition. These rules are presented as follows.
\begin{enumerate}
	\item $(\vec{s}_1, t, \vec{s}_2) \ne (\vec{t}_1, t, \vec{t}_2) \Rightarrow (\vec{s}_1, \vec{s}_2) \ne (\vec{t}_1, \vec{t}_2)$, 
		where $t \in \operatorname{T}_{\Sigma}$
	\item $(\vec{s}_1, f(\vec{s}), \vec{s}_2) \ne (\vec{t}_1, g(\vec{t}), \vec{t}_2) \Rightarrow \top$, 
		where $f \ne g \in \operatorname{Fn}$
	\item $(\vec{s}_1, t, \vec{s}_2) \ne (\vec{t}_1, x, \vec{t}_2) \Rightarrow (\vec{s}_1, \vec{s}_2) \ne (\vec{t}_1, \vec{t}_2)\sigma$, 
		where $t \in \operatorname{T}_{\Sigma}$, $\sigma = \{ x \gets t\}$
	\setcounter{enumi}{8}
	\item $(\vec{s}_1, f(\vec{s}), \vec{s}_2) \ne (\vec{t}_1, f(\vec{t}), \vec{t}_2) \Rightarrow (\vec{s}_1, \vec{s}, \vec{s}_2) \ne (\vec{t}_1, \vec{t}, \vec{t}_2)$, 
		where $f \in \operatorname{Fn}$
\end{enumerate}
It is easy to see that this extension preserves all properties of the original transformation, \ie it preserves solutions, runs in polynomial time, and 
preserves the variable disjointness of the left-hand and right-hand sides of the disequations.
%
\paragraph{Operations.}
In Section 2, the operations conjunction, difference and checking emptiness were formulated in a generic way. 
In particular, the properties of the {\mEPR} fragment were not exploited, thus, the same definitions and the 
relevant proofs are still valid. 

Furthermore, it is either easy to see that the complexity results still hold, or the referred articles handled the 
more general case with function symbols in the first place.

Finally, we note that our proposed solution for computing difference 
relies only on Remark~\ref{a-inducedsubst-remark}, which still holds. 
However, while eliminating the so-called free variables through grounding over $\mDomain$ 
is still a valid option, grounding might be even more expensive when done in a naive way.
%
\paragraph{Trail.}
Again, the definitions for the model representation and the trail can be extended in a straightforward manner, using 
the already extended corresponding syntactic and semantic notions in the new definitions.
This also includes the induced ordering. 

All relevant properties of the model representation, trail and induced ordering still hold.
We note that strictly extending a sound trail eventually terminates, as $\mathcal{A}_{\Sigma}$ is still finite.
%

==> app/s1-nc/ss-prelim.tex <==
%Non-cyclic preliminaries
We first extend our language with function symbols and sorts. 
We assume the signature $\Sigma$ contains an additional non-empty set $\mathcal{S}$ which
is made up of finitely many sort symbols.
These symbols, usually $\tau$ or $\tau_i$ in notations, denote disjoint non-empty subsets of the universe, \ie of the domain of the interpretations.
We furthermore allow the presence of non-constant function symbols, usually denoted by $f, g, h, f_i$.

We assume that each symbol has sorting information attached to, \ie for every constant and variable a sort $\tau$ is selected, and for every 
function $f$ and predicate symbol $P$ of arity $k$, we assume a given sort declaration 
$f: \tau_1 \times \tau_2 \times \dots \times \tau_k \rightarrow \tau$, 
and $P \subseteq \tau_1 \times \tau_2 \times \dots \times \tau_k$, respectively.

Furthermore, our syntax only considers well-sorted terms and formulas, using the standard definitions for well-sortedness. 
In particular, the sort of a term $t$ is denoted by $\operatorname{sort}(t)$, the set of terms of a sort $\tau$ over 
a variable set $X$ by $\operatorname{T}_{\tau}(X)$, $\operatorname{T}_{\tau}$ is a short-hand for 
$\operatorname{T}_{\tau}(\emptyset)$, and $\operatorname{T}_{\Sigma}$ or $\operatorname{T}$ 
denotes the set of all (well-sorted) ground terms over a signature $\Sigma$.

In this section we only consider the case when the corresponding Herbrand universe, \ie $\operatorname{T}_{\Sigma}$, is finite.
This fragment is the many-sorted generalization of the {\mEPR} fragment, and we call it the 
\emph{non-cyclic fragment} - a name introduced in~\cite{Noncyclic13}. 
We note that this fragment corresponds to the class $St_0$ in~\cite{AbadiRS10}.

\emph{Dependency graphs} offer an explicit characterization of the fragment, as shown in~\cite{Noncyclic13}. 
The nodes of the dependency graph of a signature $\Sigma$ are the elements of $\mathcal{S}$, 
and two sorts $\tau_1, \tau_2$ are connected with a directed edge 
iff there is a function $f$ whose sort is $\dots \times \tau_1 \times \dots \rightarrow \tau_2$, \ie
it has an argument of sort $\tau_1$, and its value-sort is $\tau_2$.

The clearly, the Herbrand universe of $\Sigma$ is infinite if and only if this graph contains a directed cycle.
Hence the name \emph{non-cyclic fragment}.

In the following, we retain the notation $\mDomain$ to denote the finite Herbrand universe of $\Sigma$.
An important consequence of the finiteness of $\mDomain$ is that $\mathcal{A}_{\Sigma}$ is still finite if $\Sigma$ is a finite signature.

Finally, we note that an unsorted problem can be turned into a many-sorted problem with efficient sort inference algorithms, see \eg \cite{ParadoxRef} for an example.
Furthermore, in a many-sorted signature the sorts responsible for the cycles can be identified and through a series of restricted flattenings, these cycles can be eliminated
at the cost of increased search space and formula size, see~\cite{Noncyclic13} for more details.
This way any finite model finding problem can be transformed into this fragment, but at a potentially reduced cost compared to the {\mEPR} transformation 
described in~\cite{Reduction2EPR09}.
%

==> app/s1-nc/ss-results.tex <==
% results
As the relevant sections, definitions and proofs rely on notions and 
properties we extended in the previous subsections, our key results 
extend to the new setting seamlessly.

The rules for our calculus are still well-defined and require no modification. 
Similarly, the notions of sound states, rules, and regularity are defined in the same 
way. More importantly, our results for soundness, and the key properties for 
regular runs extend immediately, as the proofs rely only on properties 
and definitions already lifted, and they do not exploit {\mEPR} properties explicitly.
%
\paragraph{Redundancy.} The definition of redundancy relies only on the definition for 
induced ordering. Thus, it remains unchanged. 

Moreover, our proof for non-redundant clause learning uses only this induced ordering and 
regularity, and thus, our key result still holds.
The same holds for the admissibility proofs, thus, all redundancy criterions covered in Section 6 are
still admissible.
%
\paragraph{Termination.} To prove termination, which leads to proving that NRCL is a decision procedure
for this fragment as well, we have to consider the same steps and theorems as in the {\mEPR} case.

Non-stuckness was proven using previous definitions for regularity and the rules of our calculus.
Thus, it lifts to our case without any issue.

Finite clause learning relies on Higman's Lemma~\cite{Higman52}, on the admissibility of subsumption, and on
the finiteness on $\mathcal{A}_{\Sigma}$. Since all these properties still hold, the theorem also holds and the
same proof can be used to show it.

Termination of the two distinct phases is also shown from regularity and its properties - all of which we already lifted. 
Finally, the termination of the calculus is simply a consequence of all these lemmas and theorems.
%
